Meta-Learning for Online Update of Recommender Systems

Online recommender systems should be always aligned with users' current interest to accurately suggest items that each user would like. Since user interest usually evolves over time, the update strategy should be flexible to quickly catch users' current interest from continuously generated new user-item interactions. Existing update strategies focus either on the importance of each user-item interaction or the learning rate for each recommender parameter, but such one-directional flexibility is insufficient to adapt to varying relationships between interactions and parameters. In this paper, we propose MeLON, a meta-learning based novel online recommender update strategy that supports two-directional flexibility. It is featured with an adaptive learning rate for each parameter-interaction pair for inducing a recommender to quickly learn users' up-to-date interest. The procedure of MeLON is optimized following a meta-learning approach: it learns how a recommender learns to generate the optimal learning rates for future updates. Specifically, MeLON first enriches the meaning of each interaction based on previous interactions and identifies the role of each parameter for the interaction; and then combines these two pieces of information to generate an adaptive learning rate. Theoretical analysis and extensive evaluation on three real-world online recommender datasets validate the effectiveness of MeLON.

==> eval_table.tex <==


% \renewcommand{\arraystretch}{0.8}% Tighter
\begin{table*}[htb!]
\scriptsize
\caption{Recommendation performance of BPR and NCF via six update methods on three datasets. The best results are marked in bold, and the second bests are underlined. Standard errors are reported inside parentheses.}
\vspace*{-0.2cm} 
\begin{tabular}{ X{0.83cm} | L{1.0cm} |X{0.83cm} X{0.83cm} X{0.83cm}| X{0.83cm} X{0.83cm} X{0.83cm} |X{0.83cm} X{0.83cm} X{0.83cm}| X{0.83cm} X{0.83cm} X{0.83cm}}\toprule
% \multicolumn{1}{c|}{Dataset} & Model                  & \,\,\,\,\,Method     &  HR@1\,($\uparrow$) &  HR@5\,($\uparrow$ & HR@10\,($\uparrow$) & \!\!NDCG@1\,($\uparrow$)\!\! & \!\!NDCG@5\,($\uparrow$)\!\! & \!\!\!NDCG@10\,($\uparrow$)\!\!\! & Time\,(s)\,($\downarrow$)\\ \midrule 
% \multicolumn{1}{c|}{Dataset} & Model                  & \,\,\,\,\,Method     &  HR@1 &  HR@5 & HR@10 & \!\!NDCG@1\!\! & \!\!NDCG@5\!\! & \!\!\!NDCG@10\!\!\! \\ \midrule 
\centering{\multirow{3}{*}{Dataset}} & \centering{\multirow{3}{*}{Method}} & \multicolumn{6}{c}{NCF}  \vline & \multicolumn{6}{c}{BPR}\\ \cline{3-14}
 & & \multicolumn{3}{c}{Hit Rate} \vline & \multicolumn{3}{c}{NDCG} \vline & \multicolumn{3}{c}{Hit Rate} \vline & \multicolumn{3}{c}{NDCG}\\ \cline{3-14} 
\rule{0pt}{2.5ex}& & @1 &  @5 & @10 & \!\!@1\!\! & \!\!@5\!\! & \!\!\!@10\!\!\! & @1 &  @5 & @10 & \!\!@1\!\! & \!\!@5\!\! & \!\!\!@10\!\!\! 
\\[-0.25ex] \midrule


\multirow{14}{*}{\rotatebox[origin=c]{90}{\makecell[c]{\quad\quad\quad\quad Amazon}}}
& \multirow{2}{*}{default}   
& 0.062 & 0.168 & 0.244 & 0.062 & 0.115 & 0.140 
& 0.094 & 0.246 & 0.339 & 0.094 & 0.172 & 0.202
\\[-1ex]
&
& (0.001)  & (0.001)  & (0.002)  & (0.001)  & (0.001)  & (0.001) 
& (0.001)  & (0.002)  & (0.003)  & (0.001)  & (0.002)  & (0.002)
\\[-0.5ex]

& \multirow{2}{*}{eALS}      
& 0.075 & 0.219 & 0.323 & 0.075 & 0.148 & 0.182 
& \textbf{0.143} & 0.327 & 0.425 & \textbf{0.143} & 0.238 & 0.270 
\\[-1ex]
&
& (0.003)  & (0.009)  & (0.014)  & (0.003)  & (0.006)  & (0.007) 
& (0.001)  & (0.002)  & (0.002)  & (0.001)  & (0.002)  & (0.002)
\\[-0.5ex]

& \multirow{2}{*}{MWNet}     
& 0.062 & 0.169 & 0.247 & 0.062 & 0.116 & 0.142 
& 0.094 & 0.244 & 0.339 & 0.094 & 0.171 & 0.201 
\\[-1ex]
&
& (0.001)  & (0.002)  & (0.005)  & (0.001)  & (0.001)  & (0.002) 
& (0.001)  & (0.001)  & (0.002)  & (0.001)  & (0.001)  & (0.001) 
\\[-0.5ex]

& \multirow{2}{*}{MetaSGD}   
& 0.056 & 0.151 & 0.214 & 0.056 & 0.104 & 0.125 
& 0.055 & 0.148 & 0.214 & 0.055 & 0.103 & 0.123 
\\[-1ex]
&
& (0.001)  & (0.003)  & (0.005)  & (0.001)  & (0.002)  & (0.003) 
& (0.000)  & (0.002)  & (0.005)  & (0.000)  & (0.001)  & (0.002) 
\\[-0.5ex]

& \multirow{2}{*}{S$^2$Meta} 
& 0.088 & 0.292 & 0.390 & 0.088 & 0.192 & 0.224 
& 0.084 & 0.270 & 0.367 & 0.084 & 0.178 & 0.210 
\\[-1ex]
&
& (0.002)  & (0.005)  & (0.007)  & (0.002)  & (0.003)  & (0.004) 
& (0.007)  & (0.029)  & (0.037)  & (0.007)  & (0.018)  & (0.021) 
\\[-0.5ex]

& \multirow{2}{*}{SML}       
& -  & -  & -  & -   & -   & -   
& 0.083 & 0.220 & 0.307 & 0.083 & 0.153 & 0.181 
\\[-1ex]
&
& \quad  & \quad  & \quad  & \quad  & \quad  & \quad
& (0.001)  & (0.001)  & (0.001)  & (0.001)  & (0.001)  & (0.001)
\\[-0.5ex]
%\cmidrule(r){2-14}
& \multirow{2}{*}{MeLON}     
& \textbf{0.122} & \textbf{0.324} & \textbf{0.519} & \textbf{0.122} & \textbf{0.225} & \textbf{0.287}
& \underline{0.128} & \textbf{0.363} & \textbf{0.506} & \underline{0.128} & \textbf{0.248} & \textbf{0.294}
\\ [-1ex]
&
& (0.023)  & (0.040)  & (0.034)  & (0.023)  & (0.031)  & (0.028) 
& (0.008)  & (0.016)  & (0.013)  & (0.008)  & (0.012)  & (0.011) 
\\[-0.5ex]\midrule


\multirow{14}{*}{\centering\rotatebox[origin=c]{90}{\makecell[c]{\quad\quad\quad\quad Adressa}}}
& \multirow{2}{*}{default}   
& 0.230 & 0.334 & 0.407 & 0.230  & 0.283  & 0.306   
& 0.208 & 0.292 & 0.359 & 0.208  & 0.250  & 0.272   
\\[-1ex]
&
& (0.003)  & (0.007)  & (0.009)  & (0.003)  & (0.005)  & (0.006) 
& (0.001)  & (0.002)  & (0.002)  & (0.001)  & (0.001)  & (0.001) 
\\[-0.5ex]

& \multirow{2}{*}{eALS}      
& \textbf{0.403} & 0.664 & 0.750 & \textbf{0.403}  & 0.542  & 0.570   
& 0.292 & 0.443 & 0.520 & 0.292  & 0.371  & 0.396   
\\[-1ex]
&
& (0.003)  & (0.006)  & (0.006)  & (0.003)  & (0.004)  & (0.004) 
& (0.003)  & (0.008)  & (0.011)  & (0.003)  & (0.006)  & (0.007)
\\[-0.5ex]

& \multirow{2}{*}{MWNet}    
& 0.225 & 0.325 & 0.392 & 0.225  & 0.276  & 0.297   
& 0.206 & 0.289 & 0.356 & 0.206  & 0.248  & 0.269   
\\[-1ex]
&
& (0.005)  & (0.009)  & (0.010)  & (0.005)  & (0.007)  & (0.007)
& (0.001)  & (0.001)  & (0.001)  & (0.001)  & (0.001)  & (0.001)
\\[-0.5ex]


& \multirow{2}{*}{MetaSGD}   
& 0.184 & 0.275 & 0.406 & 0.184  & 0.229  & 0.270   
& 0.185 & 0.276 & 0.405 & 0.185  & 0.230  & 0.271   
\\[-1ex]
&
& (0.000)  & (0.000)  & (0.002)  & (0.000)  & (0.000)  & (0.000)
& (0.001)  & (0.002)  & (0.002)  & (0.001)  & (0.001)  & (0.001)
\\[-0.5ex]

& \multirow{2}{*}{S$^2$Meta} 
& 0.170 & 0.276 & 0.396 & 0.170  & 0.221  & 0.260   
& 0.170 & 0.278 & 0.401 & 0.170  & 0.223  & 0.262   
\\[-1ex]
&
& (0.001)  & (0.016)  & (0.039)  & (0.001)  & (0.008)  & (0.015)
& (0.001)  & (0.015)  & (0.037)  & (0.001)  & (0.007)  & (0.014)
\\[-0.5ex]

& \multirow{2}{*}{SML}       
& -  & -  & -  & -   & -   & -    
& 0.201 & 0.270 & 0.330 & 0.201  & 0.235  & 0.255   
\\[-1ex]
&
& \quad  & \quad  & \quad  & \quad  & \quad  & \quad 
& (0.001)  & (0.001)  & (0.002)  & (0.001)  & (0.001)  & (0.001)
\\[-0.5ex]

& \multirow{2}{*}{\algname{}} 
& \underline{0.353} & \textbf{0.887} & \textbf{0.973} & \underline{0.353}  & \textbf{0.637}  & \textbf{0.666} 
& \textbf{0.436} & \textbf{0.877} & \textbf{0.958} & \textbf{0.436}  & \textbf{0.671}  & \textbf{0.698}   
\\[-1ex] 
&
& (0.037)  & (0.006)  & (0.002)  & (0.037)  & (0.021)  & (0.019)
& (0.010)  & (0.004)  & (0.001)  & (0.010)  & (0.007)  & (0.006) 
\\[-0.5ex]\midrule

\multirow{14}{*}{\rotatebox[origin=c]{90}{\makecell[c]{\quad\quad\quad\quad Yelp}}}
& \multirow{2}{*}{default}   
& 0.278 & 0.659 & 0.816 & 0.278  & 0.477  & 0.528 
& 0.239 & 0.600 & 0.766 & 0.239  & 0.426  & 0.480   
\\[-1ex]
&
& (0.001)  & (0.001)  & (0.002)  & (0.001)  & (0.001)  & (0.001)
& (0.001)  & (0.003)  & (0.004)  & (0.001)  & (0.002)  & (0.002)
\\[-0.5ex]

& \multirow{2}{*}{eALS}      
& 0.243 & 0.618 & 0.781 & 0.243  & 0.438  & 0.491 
& \textbf{0.282} & \textbf{0.677} & \textbf{0.831} & \textbf{0.282}  & \textbf{0.488}  & \textbf{0.538}
\\[-1ex]
&
& (0.003)  & (0.009)  & (0.014)  & (0.003)  & (0.006)  & (0.007)
& (0.001)  & (0.003)  & (0.003)  & (0.001)  & (0.002)  & (0.002) 
\\[-0.5ex]

& \multirow{2}{*}{MWNet}     
& 0.276 & 0.658 & 0.818 & 0.276  & 0.475  & 0.527 
& 0.240 & 0.603 & 0.771 & 0.240  & 0.428  & 0.483   
\\[-1ex]
&
& (0.001)  & (0.002)  & (0.005)  & (0.001)  & (0.001)  & (0.002)
& (0.000)  & (0.001)  & (0.001)  & (0.000)  & (0.000)  & (0.000)
\\[-0.5ex]

& \multirow{2}{*}{MetaSGD}   
& 0.065 & 0.207 & 0.309 & 0.065  & 0.136  & 0.169
& 0.065 & 0.209 & 0.321 & 0.065  & 0.137  & 0.174   
\\[-1ex]
&
& (0.001)  & (0.003)  & (0.005)  & (0.001)  & (0.002)  & (0.003)
& (0.000)  & (0.000)  & (0.003)  & (0.000)  & (0.000)  & (0.001)
\\[-0.5ex]

& \multirow{2}{*}{S$^2$Meta} 
& 0.154 & 0.393 & 0.525 & 0.154  & 0.277  & 0.320  
& 0.065 & 0.208 & 0.323 & 0.065  & 0.137  & 0.174   
\\[-1ex]
&
& (0.002)  & (0.005)  & (0.007)  & (0.002)  & (0.003)  & (0.004)
& (0.000)  & (0.001)  & (0.001)  & (0.000)  & (0.000)  & (0.001) 
\\[-0.5ex]

& \multirow{2}{*}{SML}       
& -  & -  & -  & -   & -   & -   
& 0.188 & 0.478 & 0.614 & 0.188  & 0.338  & 0.382   
\\[-1ex]
&
& \quad  & \quad  & \quad  & \quad  & \quad  & \quad
& (0.000)  & (0.000)  & (0.000)  & (0.000)  & (0.000)  & (0.000) 
\\[-0.5ex]

& \multirow{2}{*}{\algname{}}
& \textbf{0.325} & \textbf{0.779} & \textbf{0.923} & \textbf{0.325}  & \textbf{0.563}  & \textbf{0.610}   
& \underline{0.246} & \underline{0.619} & \underline{0.779} & \underline{0.246}  & \underline{0.439}  & \underline{0.491}   
\\[-1ex]
&
& (0.022)  & (0.052)  & (0.041)  & (0.022)  & (0.038)  & (0.034)
& (0.011)  & (0.017)  & (0.016)  & (0.011)  & (0.014)  & (0.014) 
\\[-0.5ex]\bottomrule
        
% \multirow{14}{*}{\rotatebox[origin=c]{90}{\makecell[c]{Yelp}}}                     
% & \multirow{2}{*}{default}   & 0.239 & 0.600 & 0.766 & 0.239  & 0.426  & 0.480   & 0.278 & 0.659 & 0.816 & 0.278  & 0.477  & 0.528   \\[-1ex]
% && ($\pm$0.001)  & ($\pm$0.003)  & ($\pm$0.004)  & ($\pm$0.001)  & ($\pm$0.002)  & ($\pm$0.002) \\
% & \multirow{2}{*}{eALS}      & \textbf{0.282} & \textbf{0.677} & \textbf{0.831} & \textbf{0.282}  & \textbf{0.488}  & \textbf{0.538}   & 0.243 & 0.618 & 0.781 & 0.243  & 0.438  & 0.491   \\
% && ($\pm$0.001)  & ($\pm$0.003)  & ($\pm$0.003)  & ($\pm$0.001)  & ($\pm$0.002)  & ($\pm$0.002) \\
% & \multirow{2}{*}{MWNet}     & 0.240 & 0.603 & 0.771 & 0.240  & 0.428  & 0.483   & 0.276 & 0.658 & 0.818 & 0.276  & 0.475  & 0.527   \\[-1ex]
% && ($\pm$0.000)  & ($\pm$0.001)  & ($\pm$0.001)  & ($\pm$0.000)  & ($\pm$0.000)  & ($\pm$0.000) \\
% & \multirow{2}{*}{MetaSGD}   & 0.065 & 0.209 & 0.321 & 0.065  & 0.137  & 0.174   & 0.065 & 0.207 & 0.309 & 0.065  & 0.136  & 0.169   \\[-1ex]
% && ($\pm$0.000)  & ($\pm$0.000)  & ($\pm$0.003)  & ($\pm$0.000)  & ($\pm$0.000)  & ($\pm$0.001) \\
% & \multirow{2}{*}{S$^2$Meta} & 0.065 & 0.208 & 0.323 & 0.065  & 0.137  & 0.174   & 0.154 & 0.393 & 0.525 & 0.154  & 0.277  & 0.320   \\[-1ex]
% && ($\pm$0.000)  & ($\pm$0.001)  & ($\pm$0.001)  & ($\pm$0.000)  & ($\pm$0.000)  & ($\pm$0.001) \\
% & \multirow{2}{*}{SML}       & 0.188 & 0.478 & 0.614 & 0.188  & 0.338  & 0.382   & -  & -  & -  & -   & -   & -    \\[-1ex]
% && ($\pm$0.000)  & ($\pm$0.000)  & ($\pm$0.000)  & ($\pm$0.000)  & ($\pm$0.000)  & ($\pm$0.000) \\
% & \multirow{2}{*}{\algname{}}& \underline{0.246} & \underline{0.619} & \underline{0.779} & \underline{0.246}  & \underline{0.439}  & \underline{0.491}   
% & \textbf{0.325} & \textbf{0.779} & \textbf{0.923} & \textbf{0.325}  & \textbf{0.563}  & \textbf{0.610}   \\[-1ex]
% && ($\pm$0.011)  & ($\pm$0.017)  & ($\pm$0.016)  & ($\pm$0.011)  & ($\pm$0.014)  & ($\pm$0.014) \\\midrule
         
                                
\end{tabular}
\label{Tab:online_update_performance_comparison}
\vspace*{-0.1cm}
\end{table*}






\begin{table*}[t!]
\vspace{-2mm}
\centering
\caption{KK
}\label{table:comp_methods}
\vspace{-0.1cm}
\resizebox{0.99\textwidth}{!}{
\centering
\begin{tabular}{cc|ccc|cccccc|ccc}
\toprule
\multirow{2}{*}{\textbf{Dataset}} &  \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{NN} & \multicolumn{6}{c|}{MM} & \multirow{2}{*}{CC} & \multirow{2}{*}{DD}  \\
& & \textbf{EE} & \textbf{FF} & \textbf{LINE} & \textbf{II} & \textbf{HH} & \textbf{GG} & \textbf{LL} & \textbf{KK} & \textbf{JJ} &  \\ \midrule

\multirow{3}{*}{AAA} & \textbf{aa} & 0.644$\pm$0.005 & 0.639$\pm$0.005 & 0.710$\pm$0.003 & 0.617$\pm$0.006 & 0.634$\pm$0.013 & 0.723$\pm$0.005 & \underline{0.773$\pm$0.003} & 0.758$\pm$0.002 & 0.768$\pm$0.002 & 0.784$\pm$0.006 & \textbf{0.798$\pm$0.002} & 0.937$\pm$0.003\\ 
  & \textbf{dd} & 0.618$\pm$0.007 & 0.600$\pm$0.005 & 0.772$\pm$0.004 & 0.606$\pm$0.003 & 0.648$\pm$0.016 & 0.750$\pm$0.007 & 0.809$\pm$0.006 & 0.813$\pm$0.004 & \underline{0.836$\pm$0.003} & \textbf{0.858$\pm$0.010} & 0.857$\pm$0.002 & 0.937$\pm$0.003\\ 
  & \textbf{\blp} & 0.654$\pm$0.012 & 0.679$\pm$0.008 & 0.859$\pm$0.005 & 0.634$\pm$0.007 & 0.710$\pm$0.017 & 0.822$\pm$0.008 & 0.851$\pm$0.007 & 0.877$\pm$0.004 & \underline{0.917$\pm$0.002} & \textbf{0.943$\pm$0.008} & 0.937$\pm$0.003 & 0.937$\pm$0.003\\ \midrule

\multirow{3}{*}{BBB} & \textbf{bb} & 0.890$\pm$0.002 & 0.880$\pm$0.003 & 0.864$\pm$0.007 & 0.823$\pm$0.002 & 0.871$\pm$0.008 & \underline{0.906$\pm$0.002} & 0.901$\pm$0.006 & 0.824$\pm$0.004 & 0.826$\pm$0.001 & 0.910$\pm$0.002 & \textbf{0.929$\pm$0.001} & 0.937$\pm$0.003\\ 
  & \textbf{\mlp} & 0.883$\pm$0.002 & 0.894$\pm$0.002 & 0.886$\pm$0.002 & 0.676$\pm$0.004 & 0.878$\pm$0.017 & \underline{0.905$\pm$0.005} & 0.890$\pm$0.007 & 0.891$\pm$0.002 & 0.850$\pm$0.002 & 0.918$\pm$0.003 & \textbf{0.933$\pm$0.001} & 0.937$\pm$0.003\\ 
  & \textbf{\blp} & 0.922$\pm$0.002 & 0.944$\pm$0.002 & 0.944$\pm$0.001 & 0.686$\pm$0.006 & 0.922$\pm$0.017 & 0.950$\pm$0.005 & 0.897$\pm$0.007 & \underline{0.966$\pm$0.001} & 0.917$\pm$0.002 & 0.966$\pm$0.004 & \textbf{0.971$\pm$0.001} & 0.937$\pm$0.003\\ \midrule

\multirow{3}{*}{CCC} & \textbf{cc} & 0.880$\pm$0.009 & 0.948$\pm$0.003 & 0.936$\pm$0.003 & 0.939$\pm$0.002 & 0.946$\pm$0.039 & 0.954$\pm$0.002 & \underline{0.955$\pm$0.002} & 0.951$\pm$0.002 & \underline{0.955$\pm$0.001} & 0.948$\pm$0.002 & \textbf{0.960$\pm$0.002} & 0.937$\pm$0.003\\ 
  & \textbf{\mlp} & 0.902$\pm$0.007 & 0.956$\pm$0.003 & 0.957$\pm$0.002 & 0.950$\pm$0.002 & 0.944$\pm$0.033 & 0.968$\pm$0.003 & 0.963$\pm$0.002 & 0.968$\pm$0.002 & \underline{0.971$\pm$0.002} & 0.969$\pm$0.001 & \textbf{0.976$\pm$0.001} & 0.937$\pm$0.003\\ 
  & \textbf{\blp} & 0.950$\pm$0.006 & 0.982$\pm$0.001 & 0.989$\pm$0.001 & 0.930$\pm$0.001 & 0.976$\pm$0.027 & 0.991$\pm$0.002 & 0.979$\pm$0.001 & 0.990$\pm$0.001 & \underline{0.994$\pm$0.001} & 0.994$\pm$0.001 & \textbf{0.996$\pm$0.001}& 0.937$\pm$0.003 \\ \midrule

\multirow{3}{*}{DDD} & \textbf{dd} & 0.831$\pm$0.001 & 0.832$\pm$0.002 & 0.824$\pm$0.001 & 0.772$\pm$0.001 & 0.836$\pm$0.009 & 0.839$\pm$0.004 & \underline{0.864$\pm$0.002} & 0.855$\pm$0.002 & 0.831$\pm$0.001 & 0.880$\pm$0.006 & \textbf{0.888$\pm$0.001} & 0.937$\pm$0.003\\ 
  & \textbf{\mlp} & 0.682$\pm$0.001 & 0.759$\pm$0.001 & 0.827$\pm$0.001 & 0.701$\pm$0.001 & 0.791$\pm$0.033 & 0.815$\pm$0.001 & 0.825$\pm$0.002 & \underline{0.883$\pm$0.001} & 0.860$\pm$0.001 & 0.881$\pm$0.007 & \textbf{0.889$\pm$0.001} & 0.937$\pm$0.003\\ 
  & \textbf{\blp} & 0.614$\pm$0.001 & 0.819$\pm$0.001 & 0.863$\pm$0.001 & 0.630$\pm$0.002 & 0.838$\pm$0.029 & 0.851$\pm$0.003 & 0.802$\pm$0.002 & \underline{0.915$\pm$0.001} & 0.901$\pm$0.001 & 0.917$\pm$0.006 & \textbf{0.921$\pm$0.002}& 0.937$\pm$0.003 \\ 
\bottomrule

\end{tabular}
}
\end{table*} 











% \renewcommand{\arraystretch}{0.8}% Tighter
\begin{table*}[htb!]
\caption{Recommendation performance of BPR and NCF via six update methods on three datasets with standard error. The best results are marked in bold, and the second bests are underlined. The performance of NCF under SML is not reported because SML is tailored to BPR.}
% \vspace*{-0.2cm} 
\resizebox{\textwidth}{!}{
\begin{tabular}{c|l|ccc|ccc|ccc|ccc}\toprule
\centering{\multirow{2}{*}{Dataset}} & \centering{\multirow{2}{*}{\, Method}} & \multicolumn{6}{c}{NCF}  \vline & \multicolumn{6}{c}{BPR}\\ \cline{3-14}
\rule{0pt}{2.5ex}& & HR@1 &  HR@5 & HR@10 & \!\!NDCG@1\!\! & \!\!NDCG@5\!\! & \!\!\!NDCG@10\!\!\! & HR@1 &  HR@5 & HR@10 & \!\!NDCG@1\!\! & \!\!NDCG@5\!\! & \!\!\!NDCG@10\!\!\! 
\\[-0.25ex] \midrule

\multirow{7}{*}{\rotatebox[origin=c]{90}{\makecell[c]{Amazon}}}
& Default
& 0.062$\pm$0.001 & 0.168$\pm$0.001 & 0.244$\pm$0.002 & 0.062$\pm$0.001 & 0.115$\pm$0.001 & 0.140$\pm$0.001
& 0.094$\pm$0.001 & 0.246$\pm$0.002 & 0.339$\pm$0.003 & 0.094$\pm$0.001 & 0.172$\pm$0.002 & 0.202$\pm$0.002
\\

& eALS
& 0.075$\pm$0.003 & 0.219$\pm$0.009 & 0.323$\pm$0.014 & 0.075$\pm$0.003 & 0.148$\pm$0.006 & 0.182$\pm$0.007 
& \textbf{0.143$\pm$0.001} & \underline{0.327$\pm$0.002} & \underline{0.425$\pm$0.002} & \textbf{0.143$\pm$0.001} & \underline{0.238$\pm$0.002} & \underline{0.270$\pm$0.002}
\\

& MWNet
& 0.062$\pm$0.001 & 0.169$\pm$0.002 & 0.247$\pm$0.005 & 0.062$\pm$0.001 & 0.116$\pm$0.001 & 0.142$\pm$0.002
& 0.094$\pm$0.001 & 0.244$\pm$0.001 & 0.339$\pm$0.002 & 0.094$\pm$0.001 & 0.171$\pm$0.001 & 0.201$\pm$0.001 
\\

& MetaSGD
& 0.056$\pm$0.001  & 0.151$\pm$0.003  & 0.214$\pm$0.005  & 0.056$\pm$0.001  & 0.104$\pm$0.002  & 0.125$\pm$0.003
& 0.055$\pm$0.000  & 0.148$\pm$0.002  & 0.214$\pm$0.005  & 0.055$\pm$0.000  & 0.103$\pm$0.001  & 0.123$\pm$0.002
\\

& S$^2$Meta
& \underline{0.088$\pm$0.002}  & \underline{0.292$\pm$0.005}  & \underline{0.390$\pm$0.007}  & \underline{0.088$\pm$0.002}  & \underline{0.192$\pm$0.003}  & \underline{0.224$\pm$0.004}
& 0.084$\pm$0.007  & 0.270$\pm$0.029  & 0.367$\pm$0.037  & 0.084$\pm$0.007  & 0.178$\pm$0.001  & 0.018$\pm$0.021
\\

& SML
& N/A  & N/A  & N/A  & N/A   & N/A   & N/A   
& 0.083$\pm$0.001  & 0.220$\pm$0.001  & 0.307$\pm$0.001  & 0.083$\pm$0.001  & 0.153$\pm$0.001  & 0.181$\pm$0.001
\\[0.5ex]\cline{2-14}\rule{0pt}{2ex}
& MeLON
& \textbf{0.122$\pm$0.023}  & \textbf{0.324$\pm$0.040}  & \textbf{0.519$\pm$0.034}  & \textbf{0.122$\pm$0.023}  & \textbf{0.225$\pm$0.031}  & \textbf{0.287$\pm$0.028}
& \underline{0.128$\pm$0.008}  & \textbf{0.363$\pm$0.016}  & \textbf{0.506$\pm$0.013}  & \underline{0.128$\pm$0.008}  & \textbf{0.248$\pm$0.012}  & \textbf{0.294$\pm$0.011}
\\
\midrule

\multirow{7}{*}{\centering\rotatebox[origin=c]{90}{\makecell[c]{Adressa}}}
& Default
& 0.230$\pm$0.003  & 0.334$\pm$0.007  & 0.407$\pm$0.009  & 0.230$\pm$0.003  & 0.283$\pm$0.005  & 0.306$\pm$0.006
& 0.208$\pm$0.001  & 0.292$\pm$0.002  & 0.359$\pm$0.002  & 0.208$\pm$0.001  & 0.250$\pm$0.001  & 0.272$\pm$0.001
\\

& eALS
& \textbf{0.403$\pm$0.003}  & \underline{0.664$\pm$0.006}  & \underline{0.750$\pm$0.006}  & \textbf{0.403$\pm$0.003}  & \underline{0.542$\pm$0.004}  & \underline{0.570$\pm$0.004}
& \underline{0.292$\pm$0.003}  & \underline{0.443$\pm$0.008}  & \underline{0.520$\pm$0.011}  & \underline{0.292$\pm$0.003}  & \underline{0.371$\pm$0.006} & \underline{0.396$\pm$0.007}
\\

& MWNet
& 0.225$\pm$0.005  & 0.325$\pm$0.009  & 0.392$\pm$0.010  & 0.225$\pm$0.005  & 0.276$\pm$0.007  & 0.297$\pm$0.007
& 0.206$\pm$0.001  & 0.289$\pm$0.001  & 0.356$\pm$0.001  & 0.206$\pm$0.001  & 0.248$\pm$0.001  & 0.269$\pm$0.001
\\

& MetaSGD  
& 0.184$\pm$0.000  & 0.275$\pm$0.000  & 0.406$\pm$0.002  & 0.184$\pm$0.000  & 0.229$\pm$0.000  & 0.270$\pm$0.000
& 0.185$\pm$0.001  & 0.276$\pm$0.002  & 0.405$\pm$0.002  & 0.185$\pm$0.001  & 0.230$\pm$0.001  & 0.271$\pm$0.001
\\

& S$^2$Meta
& 0.170$\pm$0.001  & 0.276$\pm$0.016  & 0.396$\pm$0.039  & 0.170$\pm$0.001  & 0.221$\pm$0.008  & 0.260$\pm$0.015
& 0.170$\pm$0.001  & 0.278$\pm$0.015  & 0.401$\pm$0.037  & 0.170$\pm$0.001  & 0.223$\pm$0.007  & 0.262$\pm$0.014
\\

& SML
& N/A  & N/A  & N/A  & N/A   & N/A   & N/A    
& 0.201$\pm$0.001  & 0.270$\pm$0.001  & 0.330$\pm$0.002  & 0.201$\pm$0.001  & 0.235$\pm$0.001  & 0.255$\pm$0.001
\\[0.5ex]\cline{2-14}\rule{0pt}{2ex}

& \algname{}
& \underline{0.353$\pm$0.037}  & \textbf{0.887$\pm$0.006}  & \textbf{0.973$\pm$0.002}  & \underline{0.353$\pm$0.037}  & \textbf{0.637$\pm$0.021}  & \textbf{0.666$\pm$0.019}
& \textbf{0.436$\pm$0.010}  & \textbf{0.877$\pm$0.004}  & \textbf{0.958$\pm$0.001}  & \textbf{0.436$\pm$0.010}  & \textbf{0.671$\pm$0.007}  & \textbf{0.698$\pm$0.006}
\\
\midrule

\multirow{7}{*}{\rotatebox[origin=c]{90}{\makecell[c]{Yelp}}}
& Default
& \underline{0.278$\pm$0.001}  & \underline{0.659$\pm$0.001}  & 0.816$\pm$0.002  & \underline{0.278$\pm$0.001}  & \underline{0.477$\pm$0.001}  & \underline{0.528$\pm$0.001}
& 0.239$\pm$0.001  & 0.600$\pm$0.003  & 0.766$\pm$0.004  & 0.239$\pm$0.001  & 0.426$\pm$0.002  & 0.480$\pm$0.002
\\

& eALS
& 0.243$\pm$0.003  & 0.618$\pm$0.009  & 0.781$\pm$0.014  & 0.243$\pm$0.003  & 0.438$\pm$0.006  & 0.491$\pm$0.007
& \textbf{0.282$\pm$0.001}  & \textbf{0.677$\pm$0.003}  & \textbf{0.831$\pm$0.003} & \textbf{0.282$\pm$0.002} &\textbf{0.488$\pm$0.002} & \textbf{0.538$\pm$0.002}
\\

& MWNet
& 0.276$\pm$0.001  & 0.658$\pm$0.002  & \underline{0.818$\pm$0.005}  & 0.276$\pm$0.001  & 0.475$\pm$0.001  & 0.527$\pm$0.002
& 0.240$\pm$0.000  & 0.603$\pm$0.001  & 0.771$\pm$0.001  & 0.240$\pm$0.000  & 0.428$\pm$0.000  & 0.483$\pm$0.000
\\

& MetaSGD
& 0.065$\pm$0.001  & 0.207$\pm$0.003  & 0.309$\pm$0.005  & 0.065$\pm$0.001  & 0.136$\pm$0.002  & 0.169$\pm$0.003
& 0.065$\pm$0.000  & 0.209$\pm$0.000  & 0.321$\pm$0.003  & 0.065$\pm$0.000  & 0.137$\pm$0.000  & 0.174$\pm$0.001
\\

& S$^2$Meta
& 0.154$\pm$0.002  & 0.393$\pm$0.005  & 0.525$\pm$0.007  & 0.154$\pm$0.002  & 0.277$\pm$0.003  & 0.320$\pm$0.004
& 0.065$\pm$0.000  & 0.208$\pm$0.001  & 0.323$\pm$0.001  & 0.065$\pm$0.000  & 0.137$\pm$0.000  & 0.174$\pm$0.001
\\

& SML
& N/A  & N/A  & N/A  & N/A   & N/A   & N/A   
& 0.188$\pm$0.000  & 0.478$\pm$0.000  & 0.614$\pm$0.000  & 0.188$\pm$0.000  & 0.338$\pm$0.000  & 0.382$\pm$0.000
\\[0.5ex]\cline{2-14}\rule{0pt}{2ex}

& \algname{}
& \textbf{0.327$\pm$0.047}  & \textbf{0.779$\pm$0.010}  & \textbf{0.923$\pm$0.003}  & \textbf{0.325$\pm$0.047}  & \textbf{0.563$\pm$0.027}  & \textbf{0.610$\pm$0.024}
& \underline{0.246$\pm$0.011}  & \underline{0.619$\pm$0.017}  & \underline{0.779$\pm$0.016}  & \underline{0.246$\pm$0.011}  & \underline{0.439$\pm$0.014} & \underline{0.491$\pm$0.014}
\\
\bottomrule
                                
\end{tabular}
\label{Tab:online_update_performance_comparison}
% \vspace*{-0.1cm}
}
\end{table*}

